Browsix: Bridging the Gap Between Unix and the Browser

Applications written to run on conventional operating systems typically depend on OS abstractions like processes, pipes, signals, sockets, and a shared file system. Porting these applications to the web currently requires extensive rewriting or hosting significant portions of code server-side because browsers present a nontraditional runtime environment that lacks OS functionality. This paper presents Browsix, a framework that bridges the considerable gap between conventional operating systems and the browser, enabling unmodified programs expecting a Unix-like environment to run directly in the browser. Browsix comprises two core parts: (1) a JavaScript-only system that makes core Unix features (including pipes, concurrent processes, signals, sockets, and a shared file system) available to web applications; and (2) extended JavaScript runtimes for C, C++, Go, and Node.js that support running programs written in these languages as processes in the browser. Browsix supports running a POSIX shell, making it straightforward to connect applications together via pipes. We illustrate Browsix's capabilities via case studies that demonstrate how it eases porting legacy applications to the browser and enables new functionality. We demonstrate a Browsix-enabled LaTeX editor that operates by executing unmodified versions of pdfLaTeX and BibTeX. This browser-only LaTeX editor can render documents in seconds, making it fast enough to be practical. We further demonstrate how Browsix lets us port a client-server application to run entirely in the browser for disconnected operation. Creating these applications required less than 50 lines of glue code and no code modifications, demonstrating how easily Browsix can be used to build sophisticated web applications from existing parts without modification.

==> background.tex <==
\section{Background - The Browser Environment}
\label{sec:background}

\pdfcomment{The goal if this section is primarily to convince the reader why Browsix is needed, not to give them comprehensive understanding required to appreciate its engineering. If the web is already good enough, why do we need Browsix? Bring forward all of the issues on the web that motivate Browsix, basically. We have parallelism, and we also have communication among processes / sharing data with processes.}

% background of the current browser environment, and why we need browsix

% event-based system
% many languages that target JS - generally all take their own approaches.
%  - there is a dualism between event-based and stack-based execution,
%    but languages/compilers need to implement their own stack-ripping
%    support.
% web workers prvide parallelism, don't naturally map onto stack-based
% approach


This section provides background on the execution model of web
browsers, exiting browser mechanisms for parallelism, and a survey of
some of the compiler systems that target JavaScript and their
limitations.

\subsection{Concurrency}

Browsers allocate an execution context each web page active in a Tab
or Window.  This execution context includes a private heap, a stack,
an event queue, along with a Document Object Model (DOM) tree.  The
DOM reflects the current structure of the web page -- if there was no
JavaScript executed the DOM would have a one to one correspondence
with the initial HTML resource that was loaded.  JavaScript code
running in this execution context has access to a set of APIs provided
in the global scope that cab be used to interact with browser
resources and manipulate the DOM.  Changes to the DOM result in the
web browser redrawing the screen, and are how the web site's program
interacts with the user.  Each script included by a web page is
executed in-order from top to bottom, which gives the developer the
opportunity to register callbacks to common events (such as clicks, or
a change in the status of the DOM).  This callback-based event loop is
similar to the APIs provided by MacOS X, Android, and Windows
Presentation Foundation.

Similar to these other platforms, all callbacks are executed serially
on a single thread of execution.  In the case of the browser,
non-JavaScript tasks like painting and object-layout computations are
also performed on this same thread.  Long running computations will
delay subsequent events, including responses to user input and
repainting.

\subsection{Web workers}

Web Workers (Workers) are part of the HTML5 specification, and are
supported by all major browsers including Chrome, Safari, Firefox and
Internet Explorer.  Workers provide a mechanism for running a
JavaScript file in a separate execution context.  This separate
execution context includes a dedicated thread of execution, stack,
isolated heap, and channel for communication with the parent.  This
communication channel, enforces shared nothing, asynchronous
communication. Once a worker is started it runs concurrently with the
parent, and can execute in parallel on multi-core hardware.  The
worker can import additional scripts and issue HTTP requests, subject
to the same-origin policy of the parent.  However, Workers have access
to a much reduced set of browser APIs, and in particular don't have
access to the page's DOM.  Workers are specified as being able to
spawn child workers, although this feature is only implemented in a
single browser at the time of publication.

Workers and parents communicate by sending messages over a channel.
These messages are by-default serialized, sent to the recipient, and
deserialized into the recipient's heap.  In addition to this object
copying, it is possible to directly transfer arrays of binary data in
an efficient, zero-copy manner.  Arrays transferred like this are
referred to as transferrable objects.  If the sender tries to
deference the buffer after transfer, an exception is raised.  This
enables the browser to maintain strong memory safety and isolation
guarantees.

\subsection{JavaScript as a Compilation Target}

There is extensive existing research and engineering work around
running non-JavaScript code in web browsers.  Doppio identified
missing abstractions and runtime services required to run conventional
programming languages in the browser and showed the efficacy of
providing these by implementing a JVM in
JavaScript~\cite{doppio:pldi14}.  Emscripten is a compiler of C and
C++ to JavaScript, based on LLVM~\cite{zakai2011emscripten}.  It
enables running a number of programs and libraries in the browser,
with an emphasis on games that feature 2D or 3D graphics.  Code
compiled with Emscripten often runs within 50-100\% the performance of
native.  A number of other languages have compilers that target
JavaScript, such as Go, Clojure, and Haskell.  These projects focus on
either creating a single JavaScript ``binary'' that controls the whole
page, or on exposing the compiled code to JavaScript as a library.
They all either disallow system calls when running in the browser, or
provide limited support for e.g. running a single instance of a
transpiled program.


An alternative compilation target to JavaScript, WebAssembly, is being
developed by an industry-wide group of browser
vendors~\cite{eich:2015wasm}.  WebAssembly defines a portable,
low-level, abstract syntax tree~\cite{elliott:2015wasm}.  This
representation will be natively parsed by browser JavaScript engines,
skipping the lexing and parsing of the full JavaScript language,
yielding a 2x improvement in compilation time for large
sites~\cite{wagner:2016wasm}.  Additionally, WebAssembly is a binary
format, yielding a 10-40\% reduction in binary
size~\cite{wagner:2016wasm}.  Finally, WebAssembly can be efficiently
converted to JavaScript and executed in browsers that don't feature
native support, allowing for compatability with today's browsers.
WebAssembly is complimentary to \Browsix{} - the process model
developed in this paper should allow a wider class of applications to
be able to be represented in WebAssembly.


==> punted.tex <==
While \Browsix{} was encouraged by the success of the microkernels, the
level of abstraction available in the browser makes it hard to
directly benefit from much microkernel research and engineering.  The
L4 family of microkernels, including the formally verified seL4, owe
their success to their focus on performance, with the original version
of L4 implemented entirely in assembly~\cite{elphinstone2013l3}.
As \Browsix{} is built on top of browser abstractions, rather than
hardware, we can't achieve the same level of control and performance
in current browsers.  After Shared Array Buffers are
standardized~\cite{tc39:2016sab}, it will be worth reconsidering this,
as synchronous message passing and concepts like virtual registers
become viable.

\subsection{Web Concurrency and Parallelism}

There is work-in-progress on both instruction-level parallelism and
shared-memory parallelism in browsers today.  Google, Intel and
Mozilla are developing SIMD.js to expose single-instruction, multiple-
data operations in a uniform way across a variety of architectures,
with fallbacks on platforms lacking hardware
support~\cite{counts:2014simd}.  Shared-memory parallelism is coming
to browsers in the form of
\texttt{SharedArrayBuffer}s~\cite{herman:2015paralleljs}, allowing web
developers to opt-in to all of the benefits and drawbacks of shared
memory.  \texttt{SharedArrayBuffer}s enable a single region of memory
to be shared between Web Workers, and provide atomic operations and
synchronization primitives.  Emscripten has implemented
standards-compliant pthreads support on top of Web Workers
\texttt{SharedArrayBuffer}s.

As case studies, we implement a number of applications on top of \Browsix{}. These include a face recognition application, porting , 
Using \Browsix{} greatly simplifies the creation of sophisticated web
applications: we demonstrate \Browsix{}'s flexibility and
functionality

 enables the rapid creation of sophisticated applications within the browser;
in a series of case studies, we show how \Browsix{} makes it simp
This comibination 
parallel data processing pipelines, exploit parallelism in a realtime
computer vision task, and run an existing, mature SAT solver in the
browser without code changes. Through these case studies, we
demonstrate that
\Browsix{} applications are responsive, enable significant savings
by offloading traditional cloud tasks to user's computing devices, and 
% I use facilitate too much.
can be composed to facilitate code re-use.



The remainder of this paper is organized as follows. We first present a
brief overview of how \Browsix{} brings Unix applications into the
browser~(\S\ref{sec:overview}), and .  We then
describe the architecture of \Browsix{}, and how it maps low-level
Unix primitives onto high-level browser
abstractions~(\S\ref{sec:browsix}).  We also detail how we extend
Emscripten, GopherJS, and Node.js with \Browsix{} support, letting
previously unsupported C, C++, Go, and Node.js programs run in the
browser~(\S\ref{sec:integrations}).  We demonstrate \Browsix{}'s
utility with case studies, and . 

\begin{comment}
Many web developers avoid using Web Workers because they are restrictive and difficult to use. %!!!jwv: This is opinion; can we get facts to bolster it?
To communicate between the main browser context and a worker, a developer has to design their own message-based protocol and write message processing logic on both ends.
%!!!jwv: What about IndexedDB; can the DB be open on both worker and main app?
If the main browser context and worker need to share state, the developer needs to add messages to the protocol that keep state in sync in both the worker and the main browser context.
Most browsers do not support spawning sub-workers from workers, called \emph{nested workers}, and have not added support for them since they were first proposed in 2009.
Thus, if a worker needs to perform a task in parallel, it must delegate the request to the main browser thread, and proxy all messages to that worker through the main browser thread.
}



\begin{comment}
\subsection{\Browsix{} Execution}

Like traditional kernels, the \Browsix{} kernel is passive, executing
in response to system calls from processes, or events from the browser
or non-\Browsix{} JavaScript (analogous to hardware events or
interrupts).

\paragraph{Startup}

Upon boot, \Browsix{} initializes its internal resources, including
the filesystem.  As the BrowserFS filesystem may load multiple remote
resources, such as a zip file or a JSON file describing the directory
hierarchy, the boot process may take an arbitrary amount of time.
When complete, the user provided callback is executed to ensure the
developer doesn't attempt to access a partially-initialized kernel.

\paragraph{HTTP requests}

\Browsix{} is able to route HTTP requests to processes running in Web
Workers.  It does this by taking an object representing the request
from JavaScript and marshaling the request into an ArrayBuffer that
has the request properly formatted as an HTTP 1.1
message~\cite{rfc7230}.  The kernel then creates a socket and connects
it to the server's socket that is listening on port 8080.  The HTTP
message is sent, and the server's HTTP response is parsed into an
XMLHttpRequest response, just as the developer would see from a remote
response.  Finally their callback is invoked.

\paragraph{System Calls}

% system calls are async messages, and we rely on existing tools'
% stack ripping support.

Our \Browsix{} meme service process issues a number of system calls to
read data from disk and respond to HTTP requests.  \Browsix{} system
calls are asynchronous -- when the response is received over the
message passing channel from the server, a callback is invoked.  The
existing GopherJS system takes care of saving and restoring program
stacks - we use a blocking Go channel to pass the system call results
back to the Go program.
\end{comment}


\begin{figure}[!t]
\centering
\epsfig{file=img/utilities.eps, height=3in}
\caption{Utilities implemented for \Browsix{} were designed to run in 2
  execution environments - node.js on a traditional OS, as well as in
  a browser through \texttt{browser-node} and the Browsix kernel.}
\label{figure:nodeshell}
\end{figure}


\begin{figure}[!t]
\centering
\epsfig{file=img/utilities.eps, height=3in}
\caption{Utilities implemented for \Browsix{} were designed to run in 2
  execution environments - node.js on a traditional OS, as well as in
  a browser through \texttt{browser-node} and the Browsix kernel.}
\label{figure:nodeshell}
\end{figure}



To understand how \Browsix{}'s performance compares to the underlying
message-passing primitives the browser provides, we compare the
performance of invoking the simplest system call, \texttt{getpid}, in
various runtimes against the simplest possible Web Worker message
passing implementation.  Figure~\ref{fig:getpid_latency} shows the
overhead \Browsix{}'s syscall abstraction exhibits when integrated
with different runtimes, compared to the baseline of a ping-pong Web
Worker that replies to messages as fast as it can.  \texttt{getpid} is the
cheapest system call -- it simply looks up the integer representing the
process's ID on the kernel's Task structure and returns it.  This
system call is cheap on traditional operating systems, it consists of
switching the CPU's protection domain and several memory dereferences
-- no page tables need to be invalidated nor the scheduler invoked.
However in \Browsix{}, system calls involve message passing between
two OS-level threads, scheduling, and potentially additional threads
involved depending on the browser implementation.
\begin{figure}[!t]
  \centering\small\textbf{~~~~~~~~~\texttt{getpid} Latency relative to
	  Worker roundtrip time}\\[0.3em]
  \includegraphics{plots/getpid.pdf}
  \caption{
    \texttt{getpid} latency, measured against the time it takes for
    a bare-bones JavaScript program that sends messages between an
    worker and the main thread as fast as possible.  This highlights
    the overhead introduced by \Browsix{} and compile-to-JavaScript
    language runtimes.
    \label{fig:getpid_latency}
  }
\end{figure}

